SCISPACE: A Scientific Collaboration Workspace for File Systems in Geo-Distributed HPC Data Centers

Future terabit networks are committed to dramatically improving big data motion between geographically dispersed HPC data centers.The scientific community takes advantage of the terabit networks such as DOE's ESnet and accelerates the trend to build a small world of collaboration between geospatial HPC data centers. It improves information and resource sharing for joint simulation and analysis between the HPC data centers. In this paper, we propose to build SCISPACE (Scientific Collaboration Workspace) for collaborative data centers. It provides a global view of information shared from multiple geo-distributed HPC data centers under a single workspace. SCISPACE supports native data-access to gain high-performance when data read or write is required in native data center namespace. It is accomplished by integrating a metadata export protocol. To optimize scientific collaborations across HPC data centers, SCISPACE implements search and discovery service. To evaluate, we configured two geo-distributed small-scale HPC data centers connected via high-speed Infiniband network, equipped with LustreFS. We show the feasibility of SCISPACE using real scientific datasets and applications. The evaluation results show average 36\% performance boost when the proposed native-data access is employed in collaborations.

==> future.tex <==
\section{Future Work}
\label{sec:future}

\begin{comment}
We have identified several avenues for future study:

Currently, DSP uses the snapshot decision model based on the information available at the start of job. In future, we intend to extend DSP to continuous decision model that can consider dynamic workload environment and make decisions periodically. 
\end{comment}

We have identified several avenues for future study. Currently, DSP uses the snapshot decision model based on the information available at the start of job. In future, we aim to extend DSP to continuous decision model that can consider dynamic workload environment and make decisions periodically. In this study, we only considered a simple big data application workload, such as WC and GAG. However, we are considering to improve the \tbstore{} namespace to handle highly compute-intensive application types, including neural networks and machine learning applications. Currently, we implemented a centralized metadata manager. However, we are aiming for a large-scale public federations and want to implement a distributed metadata manager to ensure \tbstore{} fault tolerance.		

%	 At present, we implemented centralized metadata manager. Our experiment showed metadata scalability even if the number of data centers increases upto certain limit in private cloud. However, we are considering to implement distributed metadata manager to target the large-scale public cloud environment and to ensure \tbstore{} fault tolerance. 


==> workspace.tex <==
\subsection{Design and Implementation}
